Sensitivity of the High Altitude Water Cherenkov Detector to Sources of Multi-TeV Gamma Rays

The High Altitude Water Cherenkov (HAWC) observatory is an array of large water Cherenkov detectors sensitive to gamma rays and hadronic cosmic rays in the energy band between 100 GeV and 100 TeV. The observatory will be used to measure high-energy protons and cosmic rays via detection of the energetic secondary particles reaching the ground when one of these particles interacts in the atmosphere above the detector. HAWC is under construction at a site 4100 meters above sea level on the northern slope of the volcano Sierra Negra, which is located in central Mexico at 19 degrees N latitude. It is scheduled for completion in 2014. In this paper we estimate the sensitivity of the HAWC instrument to point-like and extended sources of gamma rays. The source fluxes are modeled using both unbroken power laws and power laws with exponential cutoffs. HAWC, in one year, is sensitive to point sources with integral power-law spectra as low as 5x10^-13 cm^-2 sec^-1 above 2 TeV (approximately 50 mCrab) over 5 sr of the sky. This is a conservative estimate based on simple event parameters and is expected to improve as the data analysis techniques are refined. We discuss known TeV sources and the scientific contributions that HAWC can make to our understanding of particle acceleration in these sources.

==> authorlist.tex <==
\author[MSU]{Udara Abeysekara}
\author[IF-UNAM]{Ruben Alfaro}
\author[UNACH]{C\'{e}sar Alvarez Ochoa}
\author[UMSNH]{Juan de Dios \'{A}lvarez Romero}
\author[UNACH]{Roberto Arceo}
\author[UMSNH]{Juan Carlos Arteaga Vel\'{a}zquez}
\author[MTU]{Hugo Alberto Ayala Solares}
\author[University of Utah]{Ahron Barber}
\author[UMD]{Brian Baughman}
\author[UPP]{Nazario Bautista-Elivar}
\author[IF-UNAM]{Ernesto Belmont}
\author[UW-Madison]{Segev BenZvi}
\author[UMD]{David Berley}
\author[INAOE]{Mauro Javier Bonilla Rosales}
\author[UMD]{James Braun}
\author[INAOE]{Alberto Carrami\~{n}ana}
\author[FCFM-BUAP]{Mario Alberto Castillo Maldonado}
\author[UMSNH]{Umberto Cotti}
\author[FCFM-BUAP]{Jorge Cotzomi}
\author[UdG]{Eduardo de la Fuente Acosta}
\author[UMSNH]{Cederik Le\'{o}n De Le\'{o}n Acu\~{n}a}
\author[PSU]{Tyce DeYoung}
\author[INAOE]{Raquel Diaz Hernandez}
\author[UW-Madison]{Juan Carlos Diaz-Velez}
\author[LANL]{Brenda Dingus}
\author[UW-Madison]{Michael DuVernois}
\author[GMU]{Robert Ellsworth}
\author[FCFM-BUAP]{Arturo Fernandez}
\author[UW-Madison]{Daniel Fiorino}
\author[IA-UNAM]{Nissim Illich Fraija}
\author[INAOE]{Aline Galindo}
\author[UdG]{Jose Luis Garcia Luna}
\author[UdG]{Guillemo Garcia Torales}
\author[IA-UNAM]{Fernando Garfias}
\author[IA-UNAM]{Maria Magdalena Gonz\'{a}lez}
\author[UMD]{Jordan Goodman}
\author[IF-UNAM]{Varlen Grabski}
\author[UW-Madison]{Zigfried Hampel-Arias}
\author[MTU]{Petra Huentemeyer}
\author[MTU]{Michelle Hui}
\author[LANL]{Asif Imran}
\author[IA-UNAM]{Arturo Iriarte}
\author[UC Irvine]{Peter Karn}
\author[University of Utah]{David Kieda}
\author[LANL]{Gerd J. Kunde}
\author[IGeof-UNAM]{Alejandro Lara}
\author[UNM]{Robert Lauer}
\author[IA-UNAM]{William Lee}
\author[GA Tech]{Dirk Lennarz}
\author[IF-UNAM]{Hermes Le\'{o}n Vargas}
\author[UMSNH]{Edgar Casimiro Linares}
\author[MSU]{Jim Linnemann}
\author[IF-UNAM]{Antonio Marinelli}
\author[FCFM-BUAP]{Oscar Martinez}
\author[UNM]{John Matthews}
\author[UAEH]{Pedro Miranda-Romagnoli}
\author[FCFM-BUAP]{Eduardo Moreno Barbosa}
\author[INAOE]{Janina Nava}
\author[ICN-UNAM]{Lukas Nellen}
\author[University of Utah]{Michael Newbold}
\author[UAEH]{Roberto Noriega-Papaqui}
\author[IA-UNAM]{Barbara Patricelli}
\author[FCFM-BUAP]{Rodrigo Pelayo}
\author[UPP]{Eucario Gonzalo P\'{e}rez P\'{e}rez}
\author[LANL]{John Pretz}
\author[INAOE]{Daniel Rosa-Gonzalez}
\author[FCFM-BUAP]{Humberto Salazar}
\author[IF-UNAM]{Andres Sandoval}
\author[UNACH]{Eli Santos Rodr\'{i}guez}
\author[UC Santa Cruz]{Michael Schneider}
\author[INAOE]{Sergiy Silich}
\author[LANL]{Gus Sinnis}
\author[UMD]{Andrew Smith}
\author[PSU]{Kathryne Sparks}
\author[University of Utah]{Wayne Springer}
\author[GA Tech]{Ignacio Taboada}
\author[UA]{Patrick Toale}
\author[MSU]{Kirsten Tollefson}
\author[INAOE]{Ibrahim Torres}
\author[MSU]{Tilan Ukwatta}
\author[UMSNH]{Luis Villase\~{n}or}
\author[UW-Madison]{Tom Weisgarber}
\author[UW-Madison]{Stefan Westerhoff}
\author[UW-Madison]{Ian Wisher}
\author[UMD]{Joshua Wood}
\author[UC Irvine]{Gaurang Yodh}
\author[LANL]{Patrick Younk}
\author[PSU]{Dmitry Zaborov}
\author[CINVESTAV]{Arnulfo Zepeda}
\author[MTU]{Hao Zhou}

\address[MSU]{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA
}
\address[IF-UNAM]{Instituto de F\'{i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de Mexico, Mexico
}
\address[UNACH]{CEFyMAP-Ciudad Universitaria Tuxtla Guti\'{e}rrez, Mexico
}
\address[UMSNH]{Universidad Michoacana de San Nicol\'{a}s de Hidalgo, Morelia, Mexico
}
\address[MTU]{Department of Physics, Michigan Technological University, Houghton, MI, USA
}
\address[University of Utah]{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA
}
\address[UMD]{Department of Physics, University of Maryland, College Park, MD, USA
}
\address[UPP]{Universidad Politecnica de Pachuca, Pachuca, Hgo, Mexico
}
\address[UW-Madison]{Department of Physics, University of Wisconsin-Madison, Madison, WI, USA
}
\address[INAOE]{Instituto Nacional de Astrof\'{i}sica, \'{O}ptica y Electr\'{o}nica, Puebla, Mexico
}
\address[FCFM-BUAP]{Facultad de Ciencias F\'{i}sico Matem\'{a}ticas, Puebla, Mexico
}
\address[UdG]{Departamento de F\'{i}sica, Centro Universitario de Ciencias Exactas e Ingenierias, Universidad de Guadalajara, Guadalajara, Mexico
}
\address[PSU]{Department of Physics, Pennsylvania State University, University Park, PA, USA
}
\address[LANL]{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA
}
\address[GMU]{School of Physics, Astronomy, and Computational Sciences, George Mason University, Fairfax, VA, USA
}
\address[IA-UNAM]{Instituto de Astronom\'{i}a, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de Mexico, Mexico
}
\address[UC Irvine]{Department of Physics and Astronomy, University of California, Irvine, Irvine, CA, USA
}
\address[IGeof-UNAM]{Instituto de Geof\'{i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de Mexico, Mexico
}
\address[UNM]{Dept of Physics and Astronomy, University of New Mexico, Albuquerque, NM, USA
}
\address[GA Tech]{Center for Relativistic Astrophysics, School of Physics - Georgia Institute of Technology Atlanta, GA, USA
}
\address[UAEH]{Universidad Autonoma del Estado de Hidalgo, Pachuca, Mexico
}
\address[ICN-UNAM]{Instituto de Ciencias Nucleares, Universidad Nacional Autonoma de Mexico, Ciudad de Mexico, Mexico
}
\address[UC Santa Cruz]{Santa Cruz Institute for Particle Physics, University of California, Santa Cruz, Santa Cruz, CA, USA
}
\address[UA]{Department of Physics \& Astronomy, University of Alabama, Tuscaloosa, AL, USA
}
\address[CINVESTAV]{Physics Department, Centro de Investigacion y de Estudios Avanzados del IPN, Mexico City, DF, Mexico
}

